A New Multipoint Symmetric Secant Method with a Dense Initial Matrix

In large-scale optimization, when either forming or storing Hessian matrices are prohibitively expensive, quasi-Newton methods are often used in lieu of Newton's method because they only require first-order information to approximate the true Hessian. Multipoint symmetric secant (MSS) methods can be thought of as generalizations of quasi-Newton methods in that they attempt to impose additional requirements on their approximation of the Hessian. Given an initial Hessian approximation, MSS methods generate a sequence of possibly-indefinite matrices using rank-2 updates to solve nonconvex unconstrained optimization problems. For practical reasons, up to now, the initialization has been a constant multiple of the identity matrix. In this paper, we propose a new limited-memory MSS method for large-scale nonconvex optimization that allows for dense initializations. Numerical results on the CUTEst test problems suggest that the MSS method using a dense initialization outperforms the standard initialization. Numerical results also suggest that this approach is competitive with both a basic L-SR1 trust-region method and an L-PSB method.

==> implementation.tex <==
\section{The Proposed MSS Method}
In this section, we present the proposed {\small MSS} method.  This method
uses a trust-region method whose subproblems are defined
using a {\small MSS} matrix.  The result is a type of limited-memory quasi-Newton trust-region
method whose approximate Hessian can be indefinite at any given iteration.  Finally, 
this section
concludes with a discussion of the computational cost
of  the proposed  method.



\subsection{Full rank assumptions}\label{fullrankS}

\subsection{Ensuring $S_k$ has full rank}\label{fullrankS}


In order for the compact formulation to exist, it must be the case
that $S_k$ has full rank so that $W=(S_k^TS_k)^{-1}$ 
in (\ref{eqn-cptB}) is well-defined.
To ensure this, the $LDL^T$ factorization
of $S_k^TS_k$ is computed to find linearly dependent columns in $S_k$.
Specifically, small diagonal elements in  $D$ 
correspond to columns of $S_k$ that are linearly dependent.  Let
$\hat{S}_k$ denote the matrix $S_k$ after removing the linearly
dependent columns. The resulting matrix $\hat{W}\defined (\hat{S}_k^T\hat{S_k})^{-1}$ is
positive definite, and thus, invertible.  This strategy is not new and
was first proposed in this context in~\cite{burdakov2017efficiently}.  For
notational simplicity, we assume that $S_k$ has linearly independent
columns for the remainder of this section because if it is not full
rank, linear dependence will be removed by this procedure.  For the proposed
{\small MSS} method, a full rank $S_k$ is used to define $\Psi_k$.

\subsection{Ensuring $\Psi_k$ has full rank}\label{fullrankPsi}
It
is also desirable that $\Psi_k$ is full rank to avoid any adverse
affects on the condition number of $B_k$.
%To see this, $B_k$ can be
%written as
%$$B_k =\tilde{B}_0+\sum_{i=1}^{2l}\hat{\lambda_i}(QU)_i (QU)_i^T
%+ \zeta_k^CP_\perp P_\perp^T,$$
%where $\tilde{B}_0$ is given by (\ref{eqn-B0}).
If $\Psi_k$ is not
full rank, then $\hat{\Lambda}$ will have at least one diagonal entry
that is close to zero (the number of small diagonal elements of $R$
will correspond to the number of small eigenvalues of $RMR^T$).  Without loss
of generality,
assume that $i$ is such that $\hat{\lambda}_i+\zeta_k\approx \zeta_k$,
i.e., $\hat{\lambda}_i\approx 0$.  In the cases when
$|\hat{\lambda}_i+\zeta_k|\approx |\zeta_k|$ is the largest or smallest
approximate eigenvalue of $B_k$ in absolute value, the condition number of $B_k$ will be
negatively affected, possibly detrimentally.  In contrast, if
$|\hat{\lambda}_j+\zeta_k|\le|\zeta_k|\le|\hat{\lambda}_{\hat{k}}+\zeta_k|$
for some $j,\hat{k}\in \{0,1,\ldots, 2\text{rank}(S)\}$ then the condition number
of $B_k$ will not be impacted.  For this reason, ensuring that $\Psi$
has full rank will help prevent unnecessary ill-conditioning.


In order to enforce that $\Psi_k$ has  full rank, we also  perform the  $LDL^T$
factorization of $\Psi_k^T\Psi_k$ to find linearly dependent
columns of $\Psi_k$, similar to the procedure to ensure that  $S_k$ is full
rank.  
\\

\subsection{$LDL^T$ and its effect on the eigendecomposition}
Using the $LDL^T$ factorization of $\Psi_k^T\Psi_k$ in lieu of the $QR$ factorization of $\Psi_k$ in Section~\ref{sec-eig}
requires redefining the  eigendecomposition of $B_k$.
The following presentation is based on~\cite{Oleg2021}.  For notational simplicity, the subscript $k$ is dropped for all matrices.

Suppose $\Pi^T\Psi^T\Psi\Pi=LDL^T$ is the $LDL^T$ factorization of $\Psi^T\Psi$ and $\Pi$ is  a permutation matrix\footnote{For the numerical
results, MATLAB's built-in
\texttt{ldl} command, which uses rook pivoting\cite{matlab,higham02}, is used.}.  Let $J$ be the  set of  indices
such that its corresponding diagonal entry in $D$ and that of it's
``pair'' is sufficiently large (see
Section \ref{sec-complex}).
Then, $$\Psi^T\Psi\approx
\Pi\L_{\dagger}D_{\dagger}L_{\dagger}^T\Pi^T=\Pi R_{\dagger}^TR_{\dagger}\Pi^T,$$
where
$L_\dagger$ is the matrix $L$ having  removed  columns indexed by an element
not in  $J$, $D_\dagger$ is the matrix $D$ having  removed any rows and columns indexed by an element not in  $J$, 
$R_\dagger \defined \sqrt{D_\dagger}L_\dagger^T\in\Re^{r\times {2l}}$, and
  $r=|J|$.  
  This gives the approximate decomposition of $B_k$:
  \begin{equation}\label{eqn-dagger}
  B_k=B_0+Q_\dagger R_\dagger \Pi^TM\Pi R_\dagger^TQ_\dagger^T,
  \end{equation}
  where $Q_\dagger\defined (\Psi\Pi)_\dagger R_\ddagger^{-1}$,
  $(\Psi\Pi)_\dagger$ is the matrix $\Psi\Pi$ having deleted columns
  not indexed in $J$, and $R_\ddagger$ is $R_{\dagger}$ having removed
  columns not indexed in $J$.  (For more details on this derivation,
  see~\cite{Oleg2021}.)

  The partial eigendecomposition proceeds as in Section~\ref{sec-eig}
  but with $R_\dagger \Pi^T M \Pi R_\dagger^T$ in lieu of $RMR^T$.
  Finally, as in~\cite{Oleg2021}, $P_\parallel$ can be computed as
  \begin{equation}\label{eqn-pparallel}P_\parallel=(\Psi\Pi)_\dagger R_\ddagger^{-1}U.\end{equation}

%Further implementation details are found in Section \ref{sec-complex}.


\subsection{The benefits of two $LDL^T$ factorizations}

While ensuring $\Psi_k$ is full rank is sufficient to identify the columns of $S_k$ that 
are linearly independent, there is a disadvantage to computing only the $LDL^T$
factorization of $\Psi_k^T\Psi_k$ in lieu of the $LDL^T$ factorizations of both of $S_k^TS_k$ and
$\Psi_k^T\Psi_k$.  Namely, using the $LDL^T$ factorization of $\Psi_k^T\Psi_k$
to identify linearly independent columns of $S_k$ has the potential of forcing the loss
of more information.  To see this, consider what occurs
when only one $LDL^T$ factorization is performed.  If the factorization
of $\Psi_k^T\Psi_k$ leads to removing a column associated with $S_k$, (e.g., the column $s_i$), then the corresponding
column of $Y_k$, (i.e., $y_i$), must also be removed in order that $S^T_kY_k$ is computable and the dimensions of $M$ are well-defined.  
Similarly, if the column of $y_i-B_0s_i$ of $\Psi_k$
needs to be removed, then to maintain dimension agreement in the compact formulation,
both $s_i$ and $y_i$ from $S_k$ and $Y_k$, respectively, must be removed to compute $M$.  In other words, columns of $\Psi_k$
must be removed in pairs.  This can lead to deleterious effects when, for example, $\Psi_k$
for a matrix of size $n\times 2l$ and
$\hat{l}$ columns are found to be linearly independent corresponding to different subscripts.  In this case, since $l$ is typically chosen to be small, potentially few columns of $\Psi_k$ may
remain; moreover, in the extreme case when $\hat{l}=l$ then
no columns of $\Psi_k$ will be preserved since columns must be removed in pairs unless additional measures are taken. 
%Not only is there loss of information in $\Psi_k$, but a second loss of information occurs
%in $M$ when columns of $S_k$ and $Y_k$ are removed from the formation of $M$.}


In contrast, performing two $LDL^T$ factorizations helps mitigate information loss.  Namely, if $s_i$ is called
upon to be removed due to the $LDL^T$ factorization of $S_k^TS_k$, it is necessary to remove $y_i$ so that  $S_k^TY_k$ can be computed. The remaining columns of $S_k$ and $Y_k$ are used to form $\Psi_k$ (and $M$).  However, if there is further dependency in $\Psi_k$, after having removed dependent columns in $S_k$, then (1) only one column needs to be removed at a time (i.e., if the column $y_i-B_0s_i$ needs to be removed, the column $s_i$ need not be removed from $\Psi_k$)
and (2)
$M$ does not need to be further altered.  To see this, consider equation~(\ref{eqn-dagger}), where columns of $\Psi_k$ are removed, $R_\dagger$ and $R_\ddagger$ are formed, and $M$ remains intact.  In other words, there is no additional information loss in $M$ when columns in $\Psi_k$ are found to be linearly dependent after
having already removed linearly dependent columns in $S_k$ (the first block of $\Psi_k$).  Thus, performing two $LDL^T$ decompositions removes the requirement that (1) columns from $\Psi_k$ are always removed in pairs and (2) mitigates additional information loss in $M$.

\subsection{MSS algorithm with a dense initial matrix}
The following algorithm is the proposed {\small MSS} algorithm.
Details follow the algorithm.  Brackets are used to denote quantities that
are stored using more than one variable.  (For example, $[Bp]=-g$
means to store $-g$ in the variable name $Bp$.)  In the below
algorithm, $m$ denotes the maximum number of stored quasi-Newton pairs
and $l$ denotes the current number of stored pairs.  The {\small MSS}
algorithm requires an initial $x$ as well as a way to compute the
function $f$ and its gradient $g$ at any point.

%% To prevent $y_i^Ts_i$ from becoming either  too large or too small for  any $i$, a quasi-Newton pair is accepted only if the following two inequalities hold:
%% \begin{eqnarray}\label{eqn-ys}
%%  | (g(x+p)-g(x))^T p| &>& \tau_1\|p\|\|g(x+p)-g(x)\|\\
%% |(g(x+p)-g(x))^Tp|&>&(1/\tau_2) \|p\|\|g(x+p)-g(x)\|,\label{eqn-ys2}
%% \end{eqnarray}
%% where $p$ is the search direction  and  $\tau_1$ and $\tau_2$ are small constants such that $0<\tau_1,\tau_2\ll 1$.


\begin{algorithm}[H]
  \begin{algorithmic}[1]%\label{alg-mss}
     \State \textbf{Input:} $x$ 
     \State Pick $0\ll \tau<\hat{\tau}$;
     \State Set $m\in [3,7]$ with $m\in\mathbb{Z}^+$, $\Delta=1$;
        \State Set $f\gets f(x)$ and $g\gets g(x)$;  $l\gets 0$;
        \State $p\gets -g$; store $[Bp]=-g$;
        	\State Use an Amijo backtracking line search to find $\alpha$;  $x\gets x+\alpha p$; 
   \State Update $f\gets f(x)$ and $g\gets g(x)$;
   \State Update $s$ and  $y$; $l\gets 1$;
   \State Update $\Delta$ using Algorithm (\ref{alg-delta});
     \WHILE{not converged} 
      \IF{$l\le m$,}
      \State {Add $s$ to $S$ and add $y$ to $Y$;  $l\gets l+1$;}
      \ELSE \State{Remove oldest pair in $S$, $Y$, and corresponding column in $\Psi$;}
      \State {Add $s$ to $S$ and add $y$ to $Y$;}
      \ENDIF
      \State {Compute $\zeta$ and $\zeta^C$ (e.g., Section \ref{parameters}); Update $\Psi$;}
    \State {Ensure $S$ and $\Psi$ are full rank using Section \ref{fullrankS}; Store $R_\dagger$, $R_\ddagger$;}
    \State{Update $M$;}
    \State {Compute the spectral decomposition $U\hat{\Lambda}U^T$ of $R_{\dagger}\Pi^T M \Pi R_{\dagger}^T$;}
    \State {$\Lambda\gets \hat{\Lambda}+\zeta I$;}
   \State {{\small$[p,Bp]$=$\text{obs}^*$($g,\Psi,R_\ddagger^{-1},U,\Lambda,\zeta,\zeta^C,\Delta$)};}
   \State {$x\gets x+p$;}
  \State  {$f\gets f(x)$ and  $g\gets g(x);$}
\State  {Update $s$ and $y$;}
\State  {Update $\Delta$ using Algorithm (\ref{alg-delta});}
\ENDWHILE
      \State  \textbf{Output:} $x$ 
 \caption{ MSS Method with dense initialization}\label{alg-mss}
\end{algorithmic}
\end{algorithm}

Algorithm \ref{alg-mss} begins by letting $B_0=I$, and thus, the
search direction is the steepest descent direction.  (Future iterations
use the dense initialization.)  The update to  $\Delta$ at each
iteration makes use of Algorithm \ref{alg-delta}, which is a standard
way to update the trust-region radius (see, for example,~\cite{nocedal2006numerical}).
In Algorithm~\ref{alg-delta},  the variable $\rho$ stores the ratio between the actual change
and the predicted change.  If this ratio is sufficiently large,
then the step is accepted and the trust-region radius is possibly updated.
If the ratio is too small, the step is rejected and $\Delta$ is decreased.
Note that the implicit update to $B_k$, i.e., the acceptance of
a new quasi-Newton pair (lines 8 and 25 in  Algorithm~\ref{alg-mss}),
is independent of whether the step is accepted in Algorithm~\ref{alg-delta}.

The $LDL^T$ decomposition is used twice in line 18 in Algorithm~\ref{alg-mss}.  Each time,
the $i$th diagonal entry of $D$ is considered to be sufficiently large provided
$$D_{ii}>\text{tol}*\max_{j}|D_{jj}|,$$
where $D_{jj}$ denotes the $j$th diagonal entry in $D$ and tol is
a small positive number (see Sections \ref{fullrankS}-\ref{fullrankPsi}
for more details).
Finally, in line  (22), a modified \texttt{obs} method (denoted
by the asterisk) is used to solve the trust-region subproblem.

\begin{algorithm}[H]
  \begin{algorithmic}[1]%\label{alg-delta}
\State \textbf{Fix:} $0<\eta_1<\eta_2<1$, $0<\gamma_1, \gamma_p<1<\gamma_2$;
    \State $\rho\gets (f_{\text{new}}-f)/(-g^Tp-0.5p^T[Bp],0)$;
    \IF{$\rho\ge\eta_1$,} 
     \State {$f\gets f_{\text{new}}$; $x\gets x+p$ and $g\gets \nabla f(x)$;}
     \IF {$\rho\ge\eta_2$,}
     \IF {$\|p\|> \gamma_p \Delta$},
     \STATE{$\Delta\gets \gamma_2\Delta$;}
     \ENDIF
             \ENDIF
      \ELSE { $\Delta\gets \gamma_1\Delta$;}
      \ENDIF
      \caption{ Update the trust-region radius}\label{alg-delta}
  \end{algorithmic}
  \end{algorithm}



\begin{theorem}\label{theorem-convergence}
  Let  $f:\Re^n\rightarrow \Re$ be a twice-continuously differentiable and
  bounded below. Suppose there exists scalars $c_1,c_2>0$ such that 
 \begin{equation}\label{Jan22-2}
 \|\nabla^2 f(x)\| \leq c_1 \quad \text{and} \quad \|B_k\| \le  c_2, 
 \end{equation}
 for all $x \in \mathbb{R}^n$ and for all $k$. Consider the sequence $\{x_k\}$ generated
 by Algorithm \ref{alg-mss} with  $\zeta, \zeta^C\in\Re$.  
Then,
$$
\lim \limits_{k \to \infty}\|\nabla f(x_k)\|=0.
$$
\end{theorem}

\begin{proof}
  Since the {\small OBS} method generates high-accuracy solutions to the
  trust-region subproblem, all the assumptions of Theorem 6.4.6 in~\cite{conn2000trust} are met, proving convergence.
%%   %requires: AF.1-AF.3, AN.1, AM.1-AM.4, AA.1
%%   %AF1 f is twice ocntinuous diffbl . done
%%   %AF2. f is boudned below.  assumed
%%   %AF.3 hessina of objective is bounded above.  assumed.
%%   %AN.1 says that something equivalnet to the two norm is used.  done
%%   %Am.1 says that the model is twice diffble.  Done.
%%   %AM.2 says that the model and objective are the same at x_k. done
%%   %AM.3 says that the gradient of  the objective and model at x_k are the same.  Done
%%   %AM 4 sys that B_k is boudned in the trust reiogn.  assumed.
%%   %  AA.1 says subproblem is solved at least as well as cauchy point.
%%   %we have this since obs solves it exactly. done
%%   %
\end{proof}
 
\subsection{Computational complexity} \label{sec-complex}
In this section, we consider the computational cost per iteration of
Algorithm (\ref{alg-mss}). 
The $LDL^T$ factorization of $S_k^TS_k$ and $\Psi_k^T\Psi_k$
are each $\mathcal{O}(l^3)$.  Moreover, if the $LDL^T$ factorization is
updated each iteration instead of computed from scratch, this cost
drops to $\mathcal{O}(l^2)$.  The spectral decomposition's dominant
cost is at most $\mathcal{O}(l^3)=\left(l^2/n\right)\mathcal{O}(nl)$, depending on the rank of $\Psi_k$.
Finally, the \texttt{obs} method requires two  matrix-vector products
with $P_\parallel$, whose dominant cost is
 $\mathcal{O}(4nl)$ flops to solve each trust-region subproblem.
(For comparison, this is the same as the dominant cost of {\small L-BFGS}~\cite{Nocedal80}.)

 %% Similar to~\cite{Oleg2021}, we do not store $\Psi_k$ explicitly;
 %% instead, we store $S$ and $Y$.  We implicilty perform matrix-vector
 %% products with $\Psi$ using matrix-vector products with $S$ and $Y$.
 %% Furthermore, in lieu of $\Psi_k^T\Psi_k$, we store $S_k^TS_k$,
 %% $Y_k^TY_k$, and $S_k^TY_k$.  Updates to $\Psi_k^T\Psi_k$ can be done
 %% implicitly by updating the small matrices $S_k^TS_k$, $Y_k^TY_k$, and
 %% $S_k^TY_k$.


